Concurrent Binary Trees for Large-Scale Game Components

A concurrent binary tree (CBT) is a GPU-friendly data-structure suitable for the generation of bisection based terrain tessellations, i.e., adaptive triangulations over square domains. In this paper, we expand the benefits of this data-structure in two respects. First, we show how to bring bisection based tessellations to arbitrary polygon meshes rather than just squares. Our approach consists of mapping a triangular subdivision primitive, which we refer to as a bisector, to each halfedge of the input mesh. These bisectors can then be subdivided adaptively to produce conforming triangulations solely based on halfedge operators. Second, we alleviate a limitation that restricted the triangulations to low subdivision levels. We do so by using the CBT as a memory pool manager rather than an implicit encoding of the triangulation as done originally. By using a CBT in this way, we concurrently allocate and/or release bisectors during adaptive subdivision using shared GPU memory. We demonstrate the benefits of our improvements by rendering planetary scale geometry out of very coarse meshes. Performance-wise, our triangulation method evaluates in less than 0.2ms on console-level hardware.

==> figures/figure-bisection-overview-adaptive-bisection.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.441363, 0.020509) {\scalebox{0.700000}{$b_{0}^{0}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (0.071739, 0.539900) -- (0.228691, 0.489270) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.180424, 0.447038) {\scalebox{0.700000}{$b_{92}^{3}$}};
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.580000, 0.480000) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.359219, 0.539244) {\scalebox{0.700000}{$b_{2}^{0}$}};
\fill[mygreylighter]
(-0.580000, 0.480000) -- (-0.715048, -0.377512) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.565113, 0.127455) {\scalebox{0.700000}{$b_{3}^{0}$}};
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.231253, -0.367386) {\scalebox{0.700000}{$b_{4}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (-0.208751, 0.159164) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.062487, -0.188494) {\scalebox{0.700000}{$b_{5}^{0}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.715048, -0.377512) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.383142, -0.151366) {\scalebox{0.700000}{$b_{6}^{0}$}};
\fill[mygreylighter]
(0.732964, -0.073733) -- (0.240842, 0.221945) -- (0.631704, 0.290801) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.535170, 0.146337) {\scalebox{0.700000}{$b_{20}^{1}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.093003, -0.035930) {\scalebox{0.700000}{$b_{8}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.406908, -0.113562) {\scalebox{0.700000}{$b_{9}^{0}$}};
\fill[mygreylighter]
(0.530444, 0.655336) -- (0.216540, 0.756595) -- (0.385643, 0.438640) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.377542, 0.616857) {\scalebox{0.700000}{$b_{44}^{2}$}};
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.153058, 0.508509) -- (0.071739, 0.539900) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.059561, 0.635421) {\scalebox{0.700000}{$b_{28}^{2}$}};
\fill[mygreylighter]
(0.071739, 0.539900) -- (0.216540, 0.756595) -- (0.228691, 0.489270) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.172323, 0.595255) {\scalebox{0.700000}{$b_{93}^{3}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (-0.208751, 0.159164) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.040322, 0.296539) {\scalebox{0.700000}{$b_{15}^{1}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.400291, 0.279877) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.254033, 0.315850) {\scalebox{0.700000}{$b_{2}^{1}$}};
\fill[mygreylighter]
(-0.400291, 0.279877) -- (-0.097365, 0.857855) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.206905, 0.548747) {\scalebox{0.700000}{$b_{3}^{1}$}};
\fill[mygreylighter]
(-0.153058, 0.508509) -- (0.240842, 0.221945) -- (0.071739, 0.539900) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.053174, 0.443451) {\scalebox{0.700000}{$b_{29}^{2}$}};
\fill[mygreylighter]
(0.216540, 0.756595) -- (-0.097365, 0.857855) -- (0.071739, 0.539900) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.063638, 0.718117) {\scalebox{0.700000}{$b_{47}^{2}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (0.631704, 0.290801) -- (0.385643, 0.438640) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.419396, 0.337129) {\scalebox{0.700000}{$b_{42}^{2}$}};
\fill[mygreylighter]
(0.631704, 0.290801) -- (0.530444, 0.655336) -- (0.385643, 0.438640) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.515931, 0.461592) {\scalebox{0.700000}{$b_{43}^{2}$}};
\fill[mygreylighter]
(0.216540, 0.756595) -- (0.385643, 0.438640) -- (0.228691, 0.489270) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.276958, 0.561502) {\scalebox{0.700000}{$b_{90}^{3}$}};
\fill[mygreylighter]
(0.385643, 0.438640) -- (0.240842, 0.221945) -- (0.228691, 0.489270) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.290059, 0.410285) {\scalebox{0.700000}{$b_{91}^{3}$}};
\draw[mygrey, line width = 0.600000, line cap = round]
(0.228691, 0.489270) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.071739, 0.539900);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.631704, 0.290801) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.732964, -0.073733) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.385643, 0.438640) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.530444, 0.655336) -- (0.216540, 0.756595);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.216540, 0.756595) -- (0.228691, 0.489270);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.228691, 0.489270) -- (0.071739, 0.539900);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.071739, 0.539900) -- (0.216540, 0.756595);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.071739, 0.539900) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (0.071739, 0.539900);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.216540, 0.756595) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.631704, 0.290801);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.385643, 0.438640) -- (0.631704, 0.290801);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.631704, 0.290801) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.216540, 0.756595) -- (0.385643, 0.438640);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.228691, 0.489270) -- (0.385643, 0.438640);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.385643, 0.438640) -- (0.240842, 0.221945);

==> figures/figure-bisection-overview-mesh.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.097365, 0.857855) -- (-0.580000, 0.480000) -- cycle;
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.208751, 0.159164) -- cycle;
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.530444, 0.655336) -- cycle;
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.584357, -0.117574) -- (-0.293236, 0.191014);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.438796, 0.036720) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.438796, 0.036720) {\scalebox{0.729000}{$h_{0}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.277794, 0.221898) -- (-0.213747, 0.623646);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.245770, 0.422772) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.245770, 0.422772) {\scalebox{0.729000}{$h_{1}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.223028, 0.631667) -- (-0.500543, 0.414400);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.361786, 0.523033) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.361786, 0.523033) {\scalebox{0.729000}{$h_{2}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.515985, 0.383516) -- (-0.593638, -0.109554);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.554812, 0.136981) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.554812, 0.136981) {\scalebox{0.729000}{$h_{3}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.507466, -0.327135) -- (0.045664, -0.391182);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.230901, -0.359159) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.230901, -0.359159) {\scalebox{0.729000}{$h_{4}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.058322, -0.377765) -- (-0.203688, -0.005130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.072683, -0.191448) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.072683, -0.191448) {\scalebox{0.729000}{$h_{5}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.227737, -0.002345) -- (-0.518858, -0.310934);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.373297, -0.156640) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.373297, -0.156640) {\scalebox{0.729000}{$h_{6}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.026678, 0.601921) -- (-0.037369, 0.200174);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.005345, 0.401048) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.005345, 0.401048) {\scalebox{0.729000}{$h_{7}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.028762, 0.166505) -- (0.233248, -0.206130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.102243, -0.019813) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.102243, -0.019813) {\scalebox{0.729000}{$h_{8}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.256790, -0.211953) -- (0.536267, 0.026767);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.396529, -0.092593) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.396529, -0.092593) {\scalebox{0.729000}{$h_{9}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.543355, 0.055373) -- (0.426906, 0.474587);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.485131, 0.264980) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.485131, 0.264980) {\scalebox{0.729000}{$h_{10}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.406148, 0.497877) -- (0.045158, 0.614326);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.225653, 0.556101) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.225653, 0.556101) {\scalebox{0.729000}{$h_{11}$}};

==> figures/figure-bisection-overview-root-bisectors.tex <==
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.441363, 0.020509) {\scalebox{0.700000}{$b_{0}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.208751, 0.159164) -- (-0.097365, 0.857855) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.235469, 0.432298) {\scalebox{0.700000}{$b_{1}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.097365, 0.857855) -- (-0.580000, 0.480000) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.359219, 0.539244) {\scalebox{0.700000}{$b_{2}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.580000, 0.480000) -- (-0.715048, -0.377512) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.565113, 0.127455) {\scalebox{0.700000}{$b_{3}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.231253, -0.367386) {\scalebox{0.700000}{$b_{4}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(0.246918, -0.488898) -- (-0.208751, 0.159164) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.062487, -0.188494) {\scalebox{0.700000}{$b_{5}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.208751, 0.159164) -- (-0.715048, -0.377512) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.383142, -0.151366) {\scalebox{0.700000}{$b_{6}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.097365, 0.857855) -- (-0.208751, 0.159164) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.021758, 0.412988) {\scalebox{0.700000}{$b_{7}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.093003, -0.035930) {\scalebox{0.700000}{$b_{8}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.406908, -0.113562) {\scalebox{0.700000}{$b_{9}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(0.732964, -0.073733) -- (0.530444, 0.655336) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.501417, 0.267849) {\scalebox{0.700000}{$b_{10}^{0}$}};
\draw[mygrey, fill = mygreylighter, line width = 0.600000, line join = round]
(0.530444, 0.655336) -- (-0.097365, 0.857855) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.224640, 0.578378) {\scalebox{0.700000}{$b_{11}^{0}$}};

==> figures/figure-compatibility-chain-1.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.441363, 0.020509) {\scalebox{0.700000}{$b_{0}^{0}$}};
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.580000, 0.480000) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.359219, 0.539244) {\scalebox{0.700000}{$b_{2}^{0}$}};
\fill[mygreylighter]
(-0.580000, 0.480000) -- (-0.715048, -0.377512) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.565113, 0.127455) {\scalebox{0.700000}{$b_{3}^{0}$}};
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.231253, -0.367386) {\scalebox{0.700000}{$b_{4}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (-0.208751, 0.159164) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.062487, -0.188494) {\scalebox{0.700000}{$b_{5}^{0}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.715048, -0.377512) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.383142, -0.151366) {\scalebox{0.700000}{$b_{6}^{0}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.093003, -0.035930) {\scalebox{0.700000}{$b_{8}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.406908, -0.113562) {\scalebox{0.700000}{$b_{9}^{0}$}};
\fill[mygreylighter]
(0.732964, -0.073733) -- (0.530444, 0.655336) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.501417, 0.267849) {\scalebox{0.700000}{$b_{10}^{0}$}};
\fill[mygreylighter]
(0.530444, 0.655336) -- (-0.097365, 0.857855) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.224640, 0.578378) {\scalebox{0.700000}{$b_{11}^{0}$}};
\fill[myorangelight]
(-0.097365, 0.857855) -- (0.240842, 0.221945) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.003194, 0.529436) {\scalebox{0.700000}{$b_{14}^{1}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (-0.208751, 0.159164) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.040322, 0.296539) {\scalebox{0.700000}{$b_{15}^{1}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.400291, 0.279877) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.254033, 0.315850) {\scalebox{0.700000}{$b_{2}^{1}$}};
\fill[mygreylighter]
(-0.400291, 0.279877) -- (-0.097365, 0.857855) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.206905, 0.548747) {\scalebox{0.700000}{$b_{3}^{1}$}};
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.530444, 0.655336) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.097365, 0.857855);

==> figures/figure-compatibility-chain-2.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.441363, 0.020509) {\scalebox{0.700000}{$b_{0}^{0}$}};
\fill[mygreylighter]
(0.530444, 0.655336) -- (0.240842, 0.221945) -- (0.216540, 0.756595) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.329275, 0.544625) {\scalebox{0.700000}{$b_{22}^{1}$}};
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.580000, 0.480000) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.359219, 0.539244) {\scalebox{0.700000}{$b_{2}^{0}$}};
\fill[mygreylighter]
(-0.580000, 0.480000) -- (-0.715048, -0.377512) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.565113, 0.127455) {\scalebox{0.700000}{$b_{3}^{0}$}};
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.231253, -0.367386) {\scalebox{0.700000}{$b_{4}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (-0.208751, 0.159164) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.062487, -0.188494) {\scalebox{0.700000}{$b_{5}^{0}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.715048, -0.377512) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.383142, -0.151366) {\scalebox{0.700000}{$b_{6}^{0}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (-0.097365, 0.857855) -- (0.216540, 0.756595) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.120006, 0.612132) {\scalebox{0.700000}{$b_{23}^{1}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.093003, -0.035930) {\scalebox{0.700000}{$b_{8}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.406908, -0.113562) {\scalebox{0.700000}{$b_{9}^{0}$}};
\fill[mygreylighter]
(0.732964, -0.073733) -- (0.530444, 0.655336) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.501417, 0.267849) {\scalebox{0.700000}{$b_{10}^{0}$}};
\fill[myorangelight]
(-0.097365, 0.857855) -- (0.240842, 0.221945) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.003194, 0.529436) {\scalebox{0.700000}{$b_{14}^{1}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (-0.208751, 0.159164) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.040322, 0.296539) {\scalebox{0.700000}{$b_{15}^{1}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.400291, 0.279877) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.254033, 0.315850) {\scalebox{0.700000}{$b_{2}^{1}$}};
\fill[mygreylighter]
(-0.400291, 0.279877) -- (-0.097365, 0.857855) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.206905, 0.548747) {\scalebox{0.700000}{$b_{3}^{1}$}};
\draw[mygrey, line width = 0.600000, line cap = round]
(0.216540, 0.756595) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.530444, 0.655336) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (0.216540, 0.756595);
%\draw[mygrey, line width = 0.600000, line cap = round]
%(0.216540, 0.756595) -- (0.240842, 0.221945);
\draw[myorange, line width = 1.200000, line cap = round, densely dashed]
(0.216540, 0.756595) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.097365, 0.857855);

==> figures/figure-compatibility-chain-3.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.441363, 0.020509) {\scalebox{0.700000}{$b_{0}^{0}$}};
\fill[mygreylighter]
(0.530444, 0.655336) -- (0.240842, 0.221945) -- (0.216540, 0.756595) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.329275, 0.544625) {\scalebox{0.700000}{$b_{22}^{1}$}};
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.580000, 0.480000) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.359219, 0.539244) {\scalebox{0.700000}{$b_{2}^{0}$}};
\fill[mygreylighter]
(-0.580000, 0.480000) -- (-0.715048, -0.377512) -- (-0.400291, 0.279877) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.565113, 0.127455) {\scalebox{0.700000}{$b_{3}^{0}$}};
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.231253, -0.367386) {\scalebox{0.700000}{$b_{4}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (-0.208751, 0.159164) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.062487, -0.188494) {\scalebox{0.700000}{$b_{5}^{0}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.715048, -0.377512) -- (-0.225627, -0.235749) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.383142, -0.151366) {\scalebox{0.700000}{$b_{6}^{0}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.093003, -0.035930) {\scalebox{0.700000}{$b_{8}^{0}$}};
\fill[mygreylighter]
(0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.406908, -0.113562) {\scalebox{0.700000}{$b_{9}^{0}$}};
\fill[mygreylighter]
(0.732964, -0.073733) -- (0.530444, 0.655336) -- (0.240842, 0.221945) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.501417, 0.267849) {\scalebox{0.700000}{$b_{10}^{0}$}};
\fill[myorangelight]
(-0.097365, 0.857855) -- (-0.153058, 0.508509) -- (0.071739, 0.539900) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.059561, 0.635421) {\scalebox{0.700000}{$b_{28}^{2}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (-0.208751, 0.159164) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.040322, 0.296539) {\scalebox{0.700000}{$b_{15}^{1}$}};
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.400291, 0.279877) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.254033, 0.315850) {\scalebox{0.700000}{$b_{2}^{1}$}};
\fill[mygreylighter]
(-0.400291, 0.279877) -- (-0.097365, 0.857855) -- (-0.153058, 0.508509) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.206905, 0.548747) {\scalebox{0.700000}{$b_{3}^{1}$}};
\fill[myorangelight]
(-0.153058, 0.508509) -- (0.240842, 0.221945) -- (0.071739, 0.539900) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.053174, 0.443451) {\scalebox{0.700000}{$b_{29}^{2}$}};
\fill[mygreylighter]
(0.240842, 0.221945) -- (0.216540, 0.756595) -- (0.071739, 0.539900) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.166373, 0.506147) {\scalebox{0.700000}{$b_{46}^{2}$}};
\fill[mygreylighter]
(0.216540, 0.756595) -- (-0.097365, 0.857855) -- (0.071739, 0.539900) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.063638, 0.718117) {\scalebox{0.700000}{$b_{47}^{2}$}};
\draw[mygrey, line width = 0.600000, line cap = round]
(0.216540, 0.756595) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.530444, 0.655336) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.225627, -0.235749) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.400291, 0.279877) -- (-0.097365, 0.857855);
\draw[myorange, line width = 1.200000, line cap = round, densely dashed]
(0.071739, 0.539900) -- (-0.153058, 0.508509);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.153058, 0.508509) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.071739, 0.539900) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.240842, 0.221945) -- (0.216540, 0.756595);
\draw[mygrey, line width = 0.600000, line cap = round]
(-0.097365, 0.857855) -- (0.071739, 0.539900);
\draw[myorange, line width = 1.200000, line cap = round, densely dashed]
(0.071739, 0.539900) -- (0.216540, 0.756595);
\draw[mygrey, line width = 0.600000, line cap = round]
(0.216540, 0.756595) -- (-0.097365, 0.857855);

==> figures/figure-halfedge-mesh.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.097365, 0.857855) -- (-0.580000, 0.480000) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.400291, 0.279877) {\scalebox{0.729000}{$f_{0}$}};
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.208751, 0.159164) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.225627, -0.215749) {\scalebox{0.729000}{$f_{1}$}};
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.530444, 0.655336) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.240842, 0.221945) {\scalebox{0.729000}{$f_{2}$}};
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.338682, 0.668927) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.338682, 0.668927) {\scalebox{0.729000}{$e_{0}$}};
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.647524, 0.051244) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.647524, 0.051244) {\scalebox{0.729000}{$e_{1}$}};
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.234065, -0.433205) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.234065, -0.433205) {\scalebox{0.729000}{$e_{2}$}};
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.461899, -0.109174) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.461899, -0.109174) {\scalebox{0.729000}{$e_{3}$}};
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.208751, 0.159164);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.153058, 0.508509) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.153058, 0.508509) {\scalebox{0.729000}{$e_{4}$}};
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.019084, -0.164867) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.019084, -0.164867) {\scalebox{0.729000}{$e_{5}$}};
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.489941, -0.281315) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.489941, -0.281315) {\scalebox{0.729000}{$e_{6}$}};
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.631704, 0.290801) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.631704, 0.290801) {\scalebox{0.729000}{$e_{7}$}};
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.216540, 0.756595) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.216540, 0.756595) {\scalebox{0.729000}{$e_{8}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.584357, -0.117574) -- (-0.293236, 0.191014);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.438796, 0.036720) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.438796, 0.036720) {\scalebox{0.729000}{$h_{0}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.277794, 0.221898) -- (-0.213747, 0.623646);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.245770, 0.422772) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.245770, 0.422772) {\scalebox{0.729000}{$h_{1}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.223028, 0.631667) -- (-0.500543, 0.414400);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.361786, 0.523033) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.361786, 0.523033) {\scalebox{0.729000}{$h_{2}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.515985, 0.383516) -- (-0.593638, -0.109554);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.554812, 0.136981) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.554812, 0.136981) {\scalebox{0.729000}{$h_{3}$}};
\draw[mygreen, line width = 0.8, ->, > = stealth, -{Latex[length = 4.000000, width = 4.000000]}]
(-0.507466, -0.327135) -- (0.045664, -0.381182);
\draw[mygreen, fill = mygreenlighter, line width = 0.8]
(-0.230901, -0.34) circle (0.06);
\node[mygreen, draw = none, anchor = center]
at (-0.230901, -0.34) {\scalebox{0.8}{$h_{4}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.058322, -0.377765) -- (-0.203688, -0.005130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.072683, -0.191448) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.072683, -0.191448) {\scalebox{0.729000}{$h_{5}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.227737, -0.002345) -- (-0.518858, -0.310934);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.373297, -0.156640) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.373297, -0.156640) {\scalebox{0.729000}{$h_{6}$}};
\draw[myblue, line width = 0.8, ->, > = stealth, -{Latex[length = 4.000000, width = 4.000000]}]
(0.026678, 0.601921) -- (-0.037369, 0.200174);
\draw[myblue, fill = mybluelighter, line width = 0.8000]
(-0.005345, 0.401048) circle (0.06000);
\node[myblue, draw = none, anchor = center]
at (-0.005345, 0.401048) {\scalebox{0.8}{$h_{7}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.028762, 0.166505) -- (0.233248, -0.206130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.102243, -0.019813) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.102243, -0.019813) {\scalebox{0.729000}{$h_{8}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.256790, -0.211953) -- (0.536267, 0.026767);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.396529, -0.092593) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.396529, -0.092593) {\scalebox{0.729000}{$h_{9}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.543355, 0.055373) -- (0.426906, 0.474587);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.485131, 0.264980) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.485131, 0.264980) {\scalebox{0.729000}{$h_{10}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.406148, 0.497877) -- (0.045158, 0.614326);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.225653, 0.556101) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.225653, 0.556101) {\scalebox{0.729000}{$h_{11}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.580000, 0.480000) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.580000, 0.480000) {\scalebox{0.729000}{$v_{0}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.097365, 0.857855) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.097365, 0.857855) {\scalebox{0.729000}{$v_{1}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.208751, 0.159164) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.208751, 0.159164) {\scalebox{0.729000}{$v_{2}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.715048, -0.377512) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.715048, -0.377512) {\scalebox{0.729000}{$v_{3}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.246918, -0.488898) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.246918, -0.488898) {\scalebox{0.729000}{$v_{4}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.732964, -0.073733) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.732964, -0.073733) {\scalebox{0.729000}{$v_{5}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.530444, 0.655336) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.530444, 0.655336) {\scalebox{0.729000}{$v_{6}$}};
